Radiative corrections to the neutral-current Drell-Yan process in the Standard Model and its minimal supersymmetric extension

An adequate description of the neutral-current Drell-Yan process at the Tevatron and the LHC, in particular, requires the inclusion of electroweak radiative corrections. We extend earlier work in this direction in various ways. First, we define and numerically compare different methods to describe the Z-boson resonance including next-to-leading order electroweak corrections; moreover, we provide explicit analytical expressions for those. Second, we pay particular attention to contributions from photon-photon and photon-quark collisions, which involve photons in the initial state, and work out how their impact can be enhanced by selection cuts. Third, we supplement the O(\alpha) corrections by universal electroweak effects of higher order, such as universal two-loop contributions from \Delta\alpha and \Delta\rho, and the leading two-loop corrections in the high-energy Sudakov regime as well as multi-photon radiation off muons in the structure-function approach. Finally, we present results on the complete next-to-leading order electroweak and QCD corrections within the minimal supersymmetric extension of the Standard Model.

==> setup.tex <==
\usepackage{graphics}
%\usepackage{amsmath}
\usepackage{feynarts2}
\usepackage{cite}
%\usepackage{axodraw}
\usepackage{rotating}
\usepackage{url}
%\usepackage{hyperref}

\hfuzz .5pt

\makeatletter
 \setlength{\clubpenalty}{10000}
 \setlength{\widowpenalty}{10000}
 \setlength{\displaywidowpenalty}{10000}

\arraycolsep 2pt
\footnotesep 14pt

\if@twoside \oddsidemargin -17pt \evensidemargin 00pt
\else \oddsidemargin 00pt \evensidemargin 00pt
\fi
\topmargin 00pt \headheight 00pt \headsep 00pt
%\footheight 12pt \footskip 30pt
\textheight 230mm \textwidth 161mm

\renewcommand{\theparagraph}{(\roman{paragraph})}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{+2.00ex plus
 +1ex minus +.2ex}{1.5ex plus .2ex}{\it\normalsize}}

%\def\section{\@startsection {section}{1}{\z@}{+3.0ex plus +1ex minus
% +.2ex}{2.3ex plus .2ex}{\normalsize\bf}}
%\def\subsection{\@startsection{subsection}{2}{\z@}{+2.5ex plus +1ex
%minus +.2ex}{1.5ex plus .2ex}{\normalsize\bf}}
%\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{+3.25ex plus
% +1ex minus +.2ex}{1.5ex plus .2ex}{\normalsize\bf}}

\expandafter\ifx\csname mathrm\endcsname\relax\def\mathrm#1{{\rm #1}}\fi

% Equation Numbering
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\newcounter{saveeqn}
\newcommand{\alpheqn}{\setcounter{saveeqn}{\value{equation}}%
   \addtocounter{saveeqn}{1} \setcounter{equation}{0}%
   \renewcommand{\theequation}%
   {{\thesection.\arabic{saveeqn}\alph{equation}}}}
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}%
   \renewcommand{\theequation}{\thesection.\arabic{equation}}}
 
\@addtoreset{equation}{section}

\makeatother

\renewcommand{\topfraction}{0.7}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.2}
\renewcommand{\floatpagefraction}{0.7}

% new commands
\def\REF#1#2{\\[-4cm] \hspace*{#1} \rlap{\vphantom{\rule{1mm}{4cm}}
        \parbox[b]{16cm}{\baselineskip 16pt{\normalsize #2}}}}
\def\co{\relax}
\def\co{,}
\def\nl{\nonumber\\}
\def\nlc{\co\nonumber\\}
\def\nln{\nonumber\\*[-1ex]\phantom{\fbox{\rule{0em}{2ex}}}}
\def\eqskipcorr{\vspace{-\abovedisplayskip}
                \vspace{\abovedisplayshortskip}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqar{\begin{eqnarray}}
\def\eeqar{\end{eqnarray}}
\def\barr#1{\begin{array}{#1}}
\def\earr{\end{array}}
\def\bfi{\begin{figure}}
\def\efi{\end{figure}}
\def\btab{\begin{table}}
\def\etab{\end{table}}
\def\bce{\begin{center}}
\def\ece{\end{center}}
\def\nn{\nonumber}
\def\disp{\displaystyle}
\def\text{\textstyle}
\def\arraystretch{1.4}

% shorthands for greek letters
\def\al{\alpha}
\def\be{\beta}
\def\ga{\gamma}
\def\de{\delta}
\def\veps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\La{\Lambda}

% new commands for cross referencing
\def\refeq#1{\mbox{(\ref{#1})}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
%\def\refta#1{\mbox{Tab.~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
%\def\reftas#1{\mbox{Tabs.~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
%\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
%\def\refapp#1{\mbox{Appendix~\ref{#1}}}
\def\refapps#1{\mbox{Apps.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}


%physical units
\newcommand{\eV}{\ensuremath{\unskip\,\mathrm{eV}}}
\newcommand{\GeV}{\ensuremath{\unskip\,\mathrm{GeV}}}
\newcommand{\MeV}{\ensuremath{\unskip\,\mathrm{MeV}}}
\newcommand{\TeV}{\ensuremath{\unskip\,\mathrm{TeV}}}
\newcommand{\fba}{\ensuremath{\unskip\,\mathrm{fb}}}
\newcommand{\mba}{\ensuremath{\unskip\,\mathrm{mb}}}
\newcommand{\pba}{\ensuremath{\unskip\,\mathrm{pb}}}
\newcommand{\nba}{\ensuremath{\unskip\,\mathrm{nb}}}

%+X in processes
\newcommand{\X}{X}

%physical particles
\def\mathswitchr#1{\relax\ifmmode{\mathrm{#1}}\else$\mathrm{#1}$\fi}
\def\mathswitchit#1{\relax\ifmmode{#1}\else$#1$\fi}
\newcommand{\PB}{\mathswitchr B}
\newcommand{\PW}{\mathswitchr W}
\newcommand{\PZ}{\mathswitchr Z}
\newcommand{\PAn}{\mathswitchr {A^0}}
\newcommand{\Pg}{\mathswitchr g}
\newcommand{\PH}{\mathswitchr H}
\newcommand{\PHgeneric}{\mathswitchr \phi^0}
\newcommand{\Pe}{\mathswitchr e}
\newcommand{\Pne}{\mathswitch \nu_{\mathrm{e}}}
\newcommand{\Pane}{\mathswitch \bar\nu_{\mathrm{e}}}
\newcommand{\Pnmu}{\mathswitch \nu_\mu}
\newcommand{\Pd}{\mathswitchr d}
%\newcommand{\Pf}{\mathswitchr f}
\newcommand{\Pf}{f}
\newcommand{\Ph}{\mathswitchr h}
\newcommand{\Pl}{l}
\newcommand{\Pu}{\mathswitchr u}
\newcommand{\Ps}{\mathswitchr s}
\newcommand{\Pb}{\mathswitchr b}
\newcommand{\Pc}{\mathswitchr c}
\newcommand{\Pt}{\mathswitchr t}
\newcommand{\Pp}{\mathswitchr p}
\newcommand{\Ppbar}{\bar{\Pp}}
\newcommand{\Pq}{\mathswitchit q}
\newcommand{\Pep}{\mathswitchr {e^+}}
\newcommand{\Pem}{\mathswitchr {e^-}}
\newcommand{\Pepm}{\mathswitchr {e^\pm}}
\newcommand{\Pmum}{\mathswitchr {\mu^-}}
\newcommand{\PWp}{\mathswitchr {W^+}}
\newcommand{\PWm}{\mathswitchr {W^-}}
\newcommand{\PWpm}{\mathswitchr {W^\pm}}
\newcommand{\PWO}{\mathswitchr {W^0}}
\newcommand{\PZO}{\mathswitchr {Z^0}}

\newcommand{\PHu}{\mathswitchr H_\Pu}
\newcommand{\PHd}{\mathswitchr H_\Pd}
\newcommand{\Phn}{\mathswitchr {h^0}}
\newcommand{\PHn}{\mathswitchr {H^0}}

% particle masses
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\newcommand{\MB}{\mathswitch {M_\PB}}
\newcommand{\Mf}{\mathswitch {m_\Pf}}
\newcommand{\Ml}{\mathswitch {m_\Pl}}
\newcommand{\Mq}{\mathswitch {m_\Pq}}
\newcommand{\MV}{\mathswitch {M_\PV}}
\newcommand{\MW}{\mathswitch {M_\PW}}
\newcommand{\hMW}{\mathswitch {\hat M_\PW}}
\newcommand{\MWpm}{\mathswitch {M_\PWpm}}
\newcommand{\MWO}{\mathswitch {M_\PWO}}
\newcommand{\MA}{\mathswitch {M_\PAn}}
\newcommand{\MZ}{\mathswitch {M_\PZ}}
\newcommand{\MH}{\mathswitch {M_\PH}}
\newcommand{\Me}{\mathswitch {m_\Pe}}
\newcommand{\Mmy}{\mathswitch {m_\mu}}
\newcommand{\Mta}{\mathswitch {m_\tau}}
\newcommand{\Md}{\mathswitch {m_\Pd}}
\newcommand{\Mu}{\mathswitch {m_\Pu}}
\newcommand{\Ms}{\mathswitch {m_\Ps}}
\newcommand{\Mc}{\mathswitch {m_\Pc}}
\newcommand{\Mb}{\mathswitch {m_\Pb}}
\newcommand{\Mt}{\mathswitch {m_\Pt}}
\newcommand{\GW}{\mathswitch {\Gamma_\PW}}

\newcommand{\Mhn}{\mathswitch {M_{\Phn}}}
\newcommand{\MHn}{\mathswitch {M_{\PHn}}}
\newcommand{\MHgeneric}{\mathswitch {M_{\PHgeneric}}}
\newcommand{\Mhntree}{\mathswitch {m_{\Phn}}}
\newcommand{\MHntree}{\mathswitch {m_{\PHn}}}

% shorthands for SM parameters
\newcommand{\scrs}{\scriptscriptstyle}
\newcommand{\sw}{\mathswitch {s_{\scrs\PW}}}
\newcommand{\cw}{\mathswitch {c_{\scrs\PW}}}
%\newcommand{\sw}{\mathswitch {s_\PW}}
%\newcommand{\cw}{\mathswitch {c_\PW}}
%\newcommand{\swbar}{\mathswitch {\bar s_\PW}}
\newcommand{\swbar}{\mathswitch {\bar s_{\scrs\PW}}}
\newcommand{\cwbar}{\mathswitch {\bar c_{\scrs\PW}}}
\newcommand{\swfbar}{\mathswitch {\bar s_{\PW,\Pf}}}
\newcommand{\swqbar}{\mathswitch {\bar s_{\PW,\Pq}}}
\newcommand{\Qf}{\mathswitch {Q_\Pf}}
\newcommand{\Ql}{\mathswitch {Q_\Pl}}
\newcommand{\Qq}{\mathswitch {Q_\Pq}}
\newcommand{\vf}{\mathswitch {v_\Pf}}
\newcommand{\af}{\mathswitch {a_\Pf}}
\newcommand{\gesi}{\mathswitch {g_\Pe}^{\sigma}}
\newcommand{\gem}{\mathswitch {g_\Pe}^-}
\newcommand{\gep}{\mathswitch {g_\Pe}^+}
\newcommand{\GF}{\mathswitch {G_\mu}}

\newcommand{\vev}{\mathswitch v}
\newcommand{\vevu}{\mathswitch v_\Pu}
\newcommand{\vevd}{\mathswitch v_\Pd}

\newcommand{\sina}{s_\alpha}
\newcommand{\cosa}{c_\alpha}
\newcommand{\sinb}{s_\beta}
\newcommand{\cosb}{c_\beta}
\newcommand{\tana}{t_\alpha}
\newcommand{\tanb}{t_\beta}
\newcommand{\cotb}{\cot \beta}

\hyphenation{brems-strah-lung}

%various shorthands
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

% slashed quantities
\newcommand{\as}{a\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\es}{\varepsilon \hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\ks}{k\hspace{-0.52em}/\hspace{0.1em}}
\newcommand{\ps}{p\hspace{-0.42em}/}%\hspace{0.1em}}
\newcommand{\qs}{q\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\hb}{h\hspace{-0.5em}\vspace{-0.3em}-\hspace{0.1em}}
\marginparwidth 1.2cm

% orders of magnitude
\newcommand{\ord}{{\cal O}}
\renewcommand{\O}{{\cal O}}
%\newcommand{\C}{{\cal C}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}

% various abbreviations
\newcommand{\rE}{{\mathrm{E}}}
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\re}{{\mathrm{e}}}
\newcommand{\ieps}{\ri\epsilon}
\newcommand{\rd}{{\mathrm{d}}}
\newcommand{\br}{{\mathrm{br}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\onel}{{\mathrm{1-loop}}}
\newcommand{\M}{{\cal {M}}}
\renewcommand{\L}{{\cal L}}
\newcommand{\F}{{\cal {F}}}
\newcommand{\bq}{{\bf q}}
\newcommand{\ehel}{\kappa}
\newcommand{\da}{\Delta\alpha}
\newcommand{\dr}{\Delta\rho}
\newcommand{\dLL}{\Delta_{\mathrm{LL}}}

\newcommand{\cut}{{\mathrm{cut}}}
\newcommand{\llog}{{\mathrm{LL}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\weak}{{\mathrm{weak}}}
\newcommand{\phot}{\ensuremath{\mathrm{phot}}}
\newcommand{\rec}{\ensuremath{\mathrm{rec}}}
\newcommand{\LO}{\ensuremath{\mathrm{LO}}}
\newcommand{\NLO}{\ensuremath{\mathrm{NLO}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\LEP}{{\mathrm{LEP}}}
\newcommand{\SLD}{{\mathrm{SLD}}}
\newcommand{\SM}{\ensuremath{\mathrm{SM}}}
\newcommand{\MSSM}{\ensuremath{\mathrm{MSSM}}}
\newcommand{\SUSY}{\ensuremath{\mathrm{SUSY}}}
\newcommand{\CM}{{\mathrm{CM}}}
\newcommand{\born}{{\mathrm{Born}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\real}{{\mathrm{real}}}
\newcommand{\sub}{{\mathrm{sub}}}
\newcommand{\ini}{{\mathrm{ini}}}
\newcommand{\fin}{{\mathrm{fin}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\nonfact}{{\mathrm{nonfact}}}
\newcommand{\res}{{\mathrm{res}}}
\newcommand{\PA}{{\mathrm{PA}}}

%my shorthands
\newcommand{\IS}{\mathrm{IS}}
\newcommand{\FS}{\mathrm{FS}}
\newcommand{\qqb}{q\bar q}
\newcommand{\llb}{l^- l^+}

\newcommand{\sprod}[2]{\langle#1\,#2\rangle}
\newcommand{\csprod}[2]{\langle#1\,#2\rangle^*}
\newcommand{\plsdist}[1]{\left[ #1 \right]_+}

\newcommand{\gqqZ}{ \ensuremath{g_{qqZ}}}
\newcommand{\gllZ}{ \ensuremath{g_{llZ}}}
\newcommand{\gffZ}{ \ensuremath{g_{ffZ}}}
\newcommand{\gqqZp}{ \ensuremath{g_{qqZ}^+}}
\newcommand{\gqqZm}{ \ensuremath{g_{qqZ}^-}}
\newcommand{\gqqZsi}{ \ensuremath{g_{qqZ}^\sigma}}
\newcommand{\gllZp}{ \ensuremath{g_{llZ}^+}}
\newcommand{\gllZm}{ \ensuremath{g_{llZ}^-}}
\newcommand{\gllZsi}{ \ensuremath{g_{llZ}^\sigma}}
\newcommand{\gffZp}{ \ensuremath{g_{ffZ}^+}}
\newcommand{\gffZm}{ \ensuremath{g_{ffZ}^-}}
\newcommand{\gffZsi}{ \ensuremath{g_{ffZ}^\sigma}}
\newcommand{\gqqA}{ \ensuremath{g_{qq\gamma}}}
\newcommand{\gllA}{ \ensuremath{g_{ll\gamma}}}
\newcommand{\gffA}{ \ensuremath{g_{ff\gamma}}}

\newcommand{\bargqqZ}{ \ensuremath{\bar g_{qqZ}}}
\newcommand{\bargllZ}{ \ensuremath{\bar g_{llZ}}}
\newcommand{\bargffZ}{ \ensuremath{\bar g_{ffZ}}}
\newcommand{\bargqqZp}{ \ensuremath{\bar g_{qqZ}^+}}
\newcommand{\bargqqZm}{ \ensuremath{\bar g_{qqZ}^-}}
\newcommand{\bargqqZsi}{ \ensuremath{\bar g_{qqZ}^\sigma}}
\newcommand{\bargllZp}{ \ensuremath{\bar g_{llZ}^+}}
\newcommand{\bargllZm}{ \ensuremath{\bar g_{llZ}^-}}
\newcommand{\bargllZsi}{ \ensuremath{\bar g_{llZ}^\sigma}}
\newcommand{\bargffZp}{ \ensuremath{\bar g_{ffZ}^+}}
\newcommand{\bargffZm}{ \ensuremath{\bar g_{ffZ}^-}}
\newcommand{\bargffZsi}{ \ensuremath{\bar g_{ffZ}^\sigma}}
\newcommand{\bargqqA}{ \ensuremath{\bar g_{qq\gamma}}}
\newcommand{\bargllA}{ \ensuremath{\bar g_{ll\gamma}}}
\newcommand{\bargffA}{ \ensuremath{\bar g_{ff\gamma}}}

\newcommand{\gqqV}{ \ensuremath{g_{qqV}}}
\newcommand{\gllV}{ \ensuremath{g_{llV}}}
\newcommand{\gqqVp}{ \ensuremath{g_{qqV}^+}}
\newcommand{\gllVp}{ \ensuremath{g_{llV}^+}}
\newcommand{\gqqVm}{ \ensuremath{g_{qqV}^-}}
\newcommand{\gllVm}{ \ensuremath{g_{llV}^-}}
\newcommand{\gffV}{ \ensuremath{g_{ffV}}}


\newcommand{\GZ}{ \ensuremath{\Gamma_\PZ}}

\newcommand{\xMZ}{\mu_\PZ}
\newcommand{\xMW}{\mu_\PW}
\newcommand{\xMT}{\Mt}
\newcommand{\xMQ}{\mathswitch {m_Q}}

\newcommand{\mypolsum}{\sum_{\sigma,\tau =\pm 1}}

\newcommand{\BoZZ}{\ensuremath{B_0(\hat s,\xMZ,\xMZ)}}
\newcommand{\Botoo}{\ensuremath{B_0(\hat t,0,0)}}
\newcommand{\Bouoo}{\ensuremath{B_0(\hat u,0,0)}}
\newcommand{\BoWW}{\ensuremath{B_0(\hat s,\xMW,\xMW)}}
\newcommand{\Boot}{\ensuremath{B_0(\hat t,0,\xMT)}}
\newcommand{\BooQ}{\ensuremath{B_0(\hat t,0,\xMQ)}}
\newcommand{\Bosoo}{\ensuremath{B_0(\hat s,0,0)}}
\newcommand{\BosoZ}{\ensuremath{B_0(\hat s,0,\xMZ)}}
\newcommand{\BoooZ}{\ensuremath{B_0(0,0,\xMZ)}}
\newcommand{\BoooW}{\ensuremath{B_0(0,0,\xMW)}}
\newcommand{\Bostt}{\ensuremath{B_0(\hat s,\xMT,\xMT)}}
\newcommand{\BootW}{\ensuremath{B_0(0,\xMT,\xMW)}}

\newcommand{\Coxabc}{\ensuremath{C_0(0,0,x,m_0^2,m_1^2,m_2^2)}}
\newcommand{\CffxVfo}{\ensuremath{C_0(m_f^2,m_f^2,x,M_V^2,m_f^2,0)}}
\newcommand{\CffpxfVfp}{\ensuremath{C_0(m_f^2,m_{f'}^2,x,m_f^2,M_V^2,m_{f'}^2)}}

\newcommand{\CoZo}{\ensuremath{C_0(0,0,\hat s,0,\xMZ,0)}}
\newcommand{\CoWo}{\ensuremath{C_0(0,0,\hat s,0,\xMW,0)}}
\newcommand{\CoWW}{\ensuremath{C_0(0,0,\hat s,\xMW,0,\xMW)}}
\newcommand{\CoWoW}{\CoWW}
\newcommand{\CotWt}{\ensuremath{C_0(0,0,\hat s,\xMT,\xMW,\xMT)}}
\newcommand{\CoWtW}{\ensuremath{C_0(0,0,\hat s,\xMW,\xMT,\xMW)}}

%\newcommand{\CoZoZ}{\ensuremath{C(\hat s,\xMZ^2,0,\xMZ^2)}}
%\newcommand{\CotoZo}{\ensuremath{C(\hat t,0,\xMZ^2,0)}}
%\newcommand{\CouoZo}{\ensuremath{C(\hat u,0,\xMZ^2,0)}}
%\newcommand{\CoWQW}{\ensuremath{C(\hat s,\xMW^2,\xMQ^2,\xMW^2)}}
%\newcommand{\CotWo}{\ensuremath{C(\hat t,\xMT^2,\xMW^2,0)}}
%\newcommand{\CoQWo}{\ensuremath{C(\hat t,\xMQ^2,\xMW^2,0)}}
%\newcommand{\Cosoeo}{\ensuremath{C^\ga_{l}(\hat s)}}
%\newcommand{\Cosofo}{\ensuremath{C^\ga_{q}(\hat s)}}
%\newcommand{\CosZeo}{\ensuremath{C^\PZ_{l}(\hat s)}}
%\newcommand{\CosZfo}{\ensuremath{C^\PZ_{q}(\hat s)}}
%\newcommand{\Coteof}{\ensuremath{C^\ga_{lq}(\hat t)}}
%\newcommand{\Coueof}{\ensuremath{C^\ga_{lq}(\hat u)}}
\newcommand{\CotlqVpQ}{\ensuremath{C_0(\Ml^2,\Mq^2,\hat t,0,M_{V'},m_Q)}}
\newcommand{\CotlqVQ}{\ensuremath{C_0(\Ml^2,\Mq^2,\hat t,0,M_V,m_Q)}}

% \newcommand{\DoxVoVpo}{\ensuremath{D_0(0,0,0,0,\hat s,x,M_{V}^2,m_Q^2,M_{V'}^2,0)}}
% \newcommand{\DoxVeof}{\ensuremath{D_0(\Ml^2,\Ml^2,\Mq^2,\Mq^2,\hat s,x,M_{V}^2,\Ml^2,0,\Mq^2)}}

% \newcommand{\DotZoZo}{\ensuremath{D^{\PZ\PZ}(\hat s,\hat t,0)}}
% \newcommand{\DouZoZo}{\ensuremath{D^{\PZ\PZ}(\hat s,\hat u,0)}}
% \newcommand{\DoWW}{   \ensuremath{D^{\PW\PW}(\hat s,\hat u,0)}}
% \newcommand{\DoWtWo}{ \ensuremath{D^{\PW\PW}(\hat s,\hat u,\xMT^2)}}
% \newcommand{\DoWQWo}{ \ensuremath{D^{\PW\PW}(\hat s,\hat u,\xMQ^2)}}
% \newcommand{\Dotoeof}{\ensuremath{D^\ga(\hat s,\hat t)}}
% \newcommand{\Douoeof}{\ensuremath{D^\ga(\hat s,\hat u)}}
% \newcommand{\DotZeof}{\ensuremath{D^\PZ(\hat s,\hat t)}}
% \newcommand{\DouZeof}{\ensuremath{D^\PZ(\hat s,\hat u)}}

\newcommand{\CoxlqVQ}{\ensuremath{C_0(\Ml^2,\Mq^2,x,0,M_V^2,m_Q^2)}}
\newcommand{\CoulqVQ}{\ensuremath{C_0(\Ml^2,\Mq^2,\hat u,0,M_V^2,m_Q^2)}}
\newcommand{\CoxlqVpQ}{\ensuremath{C_0(\Ml^2,\Mq^2,x,0,M_{V'}^2,m_Q^2)}}
\newcommand{\CoulqVpQ}{\ensuremath{C_0(\Ml^2,\Mq^2,\hat u,0,M_{'V},m_Q)}}

\newcommand{\CosqVVpQ}{\ensuremath{C_0(m_q^2,m_q^2,\hat s,M_V,m_Q,M_{V'})}}
\newcommand{\CoslVVpQ}{\ensuremath{C_0(m_l^2,m_l^2,\hat s,M_V,m_l,M_{V'})}}

\newcommand{\DoxlqVQVpo}{\ensuremath{D_0(\Mq^2,\Mq^2,\Ml^2,\Ml^2,\hat s,x,M_{V}^2,m_Q^2,M_{V'}^2,0)}}
\newcommand{\DoxlqVQVpl}{\ensuremath{D_0(\Mq^2,\Mq^2,\Ml^2,\Ml^2,\hat s,x,M_{V}^2,m_Q^2,M_{V'}^2,\Ml^2)}}

\newcommand{\DotlqVQVpo}{\ensuremath{D_0(\Mq^2,\Mq^2,\Ml^2,\Ml^2,\hat s, \hat t,M_V,m_Q,M_{V'},\Ml)}}


\newcommand{\Ord}[1]{\mathcal{O}(#1)}

% mathematical functions
\def\atn{\mathop{\mathrm{arctan}}\nolimits}
\def\Li{\mathop{\mathrm{Li}_2}\nolimits}
\def\cLi{\mathop{{\cal L}i_2}\nolimits}
\def\Re{\mathop{\mathrm{Re}}\nolimits}
\def\Im{\mathop{\mathrm{Im}}\nolimits}
\def\sgn{\mathop{\mathrm{sgn}}\nolimits}
\def\arc{\mathop{\mathrm{arc}}\nolimits}

% modifications for drafts
\newcommand{\mpar}[1]{{\marginpar{\hbadness10000%
                      \sloppy\hfuzz10pt\boldmath\bf#1}}%
                      \typeout{marginpar: #1}\ignorespaces}
\marginparwidth 1.2cm
\marginparsep 0.2cm
\def\draftdate{\relax}
\def\mda{\relax}
\def\mua{\relax}
\def\mla{\relax}
\def\draft{
\def\thtystars{******************************}
\def\sixtystars{\thtystars\thtystars}
\typeout{}
\typeout{\sixtystars**}
\typeout{* Draft mode!
         For final version remove \protect\draft\space in source file *}
\typeout{\sixtystars**}
\typeout{}
\def\draftdate{\today}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mda{\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil$\Rightarrow$]%
                   {\boldmath$\Leftarrow $\hfil}%
                    \typeout{marginpar: $\Leftrightarrow$}\ignorespaces}
\overfullrule 5pt
\oddsidemargin -15mm
\marginparwidth 29mm
}

% change of eqnarray environment
%  Default is for left-hand side of equations to be flushleft.
%  To make them flushright, \let\@eqnsel = \hfil

\makeatletter
%\let\@eqnsel = \hfil

\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
%$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
%  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
$$\halign to \displaywidth\bgroup\hskip\@centering
  $\displaystyle\tabskip\z@{##}$\@eqnsel&\global\@eqcnt\@ne
  \hskip 2\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\arraycolsep $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\appendix{\par
 \setcounter{section}{0} \setcounter{subsection}{0}
 \def\thesection{\Alph{section}}}

\newcommand{\gtrless}
{\;\rlap{\raisebox{+.25em}{$>$}}\raisebox{-.25em}{$<$}\;}
\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}
\def\asymp#1{\;\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}\;}
\newcommand{\gl}
{\;\raisebox{.25em}{$>$}\hspace{-.75em}\raisebox{-.2em}{$<$}\;}
\def\dsl{\mathpalette\make@slash}
\def\make@slash#1#2{\setbox\z@\hbox{$#1#2$}%
  \hbox to 0pt{\hss$#1/$\hss\kern-\wd0}\box0}

\newcommand{\mycaption}[2][]{{\begin{center} \parbox{15cm}{{\bf \caption[#1]{\rm {#2}}}} \end{center} }}
%\newcommand{\mycaption}[2][kurz]{{{\bf \caption[#1]{\rm {#2}}}}}

\newcommand{\Vector}[1]{{\left( \begin{array}{c} #1 \end{array} \right) }}
\newcommand{\Matrix}[1]{{\left( \begin{array}{cc} #1 \end{array} \right) }}
\newcommand{\mr}[1]{{\mathrm{#1}}}
\renewcommand{\la}{{\mathcal L}}
\newcommand{\Pbbar}{{\bar{\Pb}}}
\newcommand{\Pdbar}{{\bar{\Pd}}}
\newcommand{\Pubar}{{\bar{\Pu}}}
\newcommand{\Pqbar}{{\bar{\Pq}}}
\newcommand{\MSbar}{\ensuremath{{\overline{\mathrm{MS}}}}}
\newcommand{\DIS}{\ensuremath{{\mathrm{DIS}}}}
\newcommand{\DRbar}{{$\overline{\mathrm{DR}}$}}

\newcommand{\comment}[1]{{\noindent {\bf (#1)}}}

\newcommand{\myplot}[9]{
\begin{picture}(0,0)(0,0)
\put(#2,#3){#4}
\begin{rotate}{#8}
\put(#5,#6){#7}
\end{rotate}
\end{picture}
\includegraphics[width=#9]{#1}
}

\makeatother

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ppZll"
%%% End: 

